Affinity-based measures of medical diagnostic test accuracy

We propose new summary measures of diagnostic test accuracy which can be used as companions to existing diagnostic accuracy measures. Conceptually, our summary measures are tantamount to the so-called Hellinger affinity and we show that they can be regarded as measures of agreement constructed from similar geometrical principles as Pearson correlation. A covariate-specific version of our summary index is developed, which can be used to assess the discrimination performance of a diagnostic test, conditionally on the value of a predictor. Nonparametric Bayes estimators for the proposed indexes are devised, theoretical properties of the corresponding priors are derived, and the performance of our methods is assessed through a simulation study. Data from a prostate cancer diagnosis study are used to illustrate our methods.

==> Latex/colors.tex <==
\usepackage{color}

\def\red#1{{\color{red} #1}}%
\def\blue#1{{\color{blue} #1}}%
\def\green#1{{\color{green} #1}}

% \newcommand{\Cexpr}[1]{\blue{\Sexpr{#1}}}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> Latex/environments.tex <==
% Theorem-like structures
\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{proposition}{Proposition}
\newtheorem{conjecture}{Conjecture}
\newtheorem{corollary}[theorem]{Corollary} 
\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> Latex/short_bib.tex <==
% To shorten the reference list use:
 \let\oldthebibliography=\thebibliography
 \let\oldendthebibliography=\endthebibliography
 \renewenvironment{thebibliography}[1]{%
   \footnotesize
   \oldthebibliography{#1}%
   \setlength{\parskip}{0mm}%
   \setlength{\itemsep}{0mm}%
 }{\oldendthebibliography}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> Latex/tools.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                      Math                                    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Calculus
\newcommand{\e}{\mathrm{e}}
\newcommand{\dif}{\ensuremath{\mathrm{d}}}
\newcommand{\nto}{\ensuremath{\underset{n \to \infty}{\rightarrow}}}
% \def\tsum{\mathop{\textstyle \sum }}
% \def\tprod{\mathop{\textstyle \prod }}
% \def\tint{\mathop{\textstyle \int}}
% Linear Algebra
\newcommand{\T}{\ensuremath{\mathrm{\scriptscriptstyle T}}}
% Bold Greek Uppercase
\usepackage{bm}
\newcommand{\Gammab}{\ensuremath{\bm\Gamma}}
\newcommand{\Deltab}{\ensuremath{\bm\Delta}}
\newcommand{\Thetab}{\ensuremath{\bm\Theta}}
\newcommand{\Lambdab}{\ensuremath{\bm\Lambda}}
\newcommand{\Xib}{\ensuremath{\bm\Xi}}
\newcommand{\Pib}{\ensuremath{\bm\Pi}}
\newcommand{\Sigmab}{\ensuremath{\bm\Sigma}}
\newcommand{\Upsilonb}{\ensuremath{\bm\Upsilon}}
\newcommand{\Phib}{\ensuremath{\bm\Phi}}
\newcommand{\Psib}{\ensuremath{\bm\Psi}}
\newcommand{\Omegab}{\ensuremath{\bm\Omega}}
% Bold Greek Lowercase
\newcommand{\alphab}{\ensuremath{\bm\alpha}}
\newcommand{\betab}{\ensuremath{\bm\beta}}
\newcommand{\gammab}{\ensuremath{\bm\gamma}}
\newcommand{\deltab}{\ensuremath{\bm\delta}}
\newcommand{\epsilonb}{\ensuremath{\bm\epsilon}}
\newcommand{\zetab}{\ensuremath{\bm\zeta}}
\newcommand{\etab}{\ensuremath{\bm\eta}}
\newcommand{\thetab}{\ensuremath{\bm\theta}}
\newcommand{\iotab}{\ensuremath{\bm\iota}}
\newcommand{\kappab}{\ensuremath{\bm\kappa}}
\newcommand{\lambdab}{\ensuremath{\bm\lambda}}
\newcommand{\mub}{\ensuremath{\bm\mu}}
\newcommand{\nub}{\ensuremath{\bm\nu}}
\newcommand{\xib}{\ensuremath{\bm\xi}}
\newcommand{\pib}{\ensuremath{\bm\pi}}
\newcommand{\rhob}{\ensuremath{\bm\rho}}
\newcommand{\sigmab}{\ensuremath{\bm\sigma}}
\newcommand{\taub}{\ensuremath{\bm\tau}}
\newcommand{\upsilonb}{\ensuremath{\bm\upsilon}}
\newcommand{\phib}{\ensuremath{\bm\phi}}
\newcommand{\chib}{\ensuremath{\bm\chi}}
\newcommand{\psib}{\ensuremath{\bm\psi}}
\newcommand{\omegab}{\ensuremath{\bm\omega}}
\newcommand{\varepsilonb}{\ensuremath{\bm\varepsilon}}
\newcommand{\varthetab}{\ensuremath{\bm\vartheta}}
\newcommand{\varpib}{\ensuremath{\bm\varpi}}
\newcommand{\varrhob}{\ensuremath{\bm\varrho}}
\newcommand{\varsigmab}{\ensuremath{\bm\varsigma}}
\newcommand{\varphib}{\ensuremath{\bm\varphi}}
% Other Bold
\newcommand{\bma}{\ensuremath{\bm a}}
\newcommand{\bmb}{\ensuremath{\bm b}}
\newcommand{\bmc}{\ensuremath{\bm c}}
\newcommand{\bmd}{\ensuremath{\bm d}}
\newcommand{\bme}{\ensuremath{\bm e}}
\newcommand{\bmf}{\ensuremath{\bm f}}
\newcommand{\bmg}{\ensuremath{\bm g}}
\newcommand{\bmh}{\ensuremath{\bm h}}
\newcommand{\bmi}{\ensuremath{\bm i}}
\newcommand{\bmj}{\ensuremath{\bm j}}
\newcommand{\bmk}{\ensuremath{\bm k}}
\newcommand{\bml}{\ensuremath{\bm l}}
\newcommand{\bmm}{\ensuremath{\bm m}}
\newcommand{\bmn}{\ensuremath{\bm n}}
\newcommand{\bmo}{\ensuremath{\bm o}}
\newcommand{\bmp}{\ensuremath{\bm p}}
\newcommand{\bmq}{\ensuremath{\bm q}}
\newcommand{\bmr}{\ensuremath{\bm r}}
\newcommand{\bms}{\ensuremath{\bm s}}
\newcommand{\bmt}{\ensuremath{\bm t}}
\newcommand{\bmu}{\ensuremath{\bm u}}
\newcommand{\bmv}{\ensuremath{\bm v}}
\newcommand{\bmw}{\ensuremath{\bm w}}
\newcommand{\bmx}{\ensuremath{\bm x}}
\newcommand{\bmy}{\ensuremath{\bm y}}
\newcommand{\bmz}{\ensuremath{\bm z}}
\newcommand{\bmA}{\ensuremath{\bm A}}
\newcommand{\bmB}{\ensuremath{\bm B}}
\newcommand{\bmC}{\ensuremath{\bm C}}
\newcommand{\bmD}{\ensuremath{\bm D}}
\newcommand{\bmE}{\ensuremath{\bm E}}
\newcommand{\bmF}{\ensuremath{\bm F}}
\newcommand{\bmG}{\ensuremath{\bm G}}
\newcommand{\bmH}{\ensuremath{\bm H}}
\newcommand{\bmI}{\ensuremath{\bm I}}
\newcommand{\bmJ}{\ensuremath{\bm J}}
\newcommand{\bmK}{\ensuremath{\bm K}}
\newcommand{\bmL}{\ensuremath{\bm L}}
\newcommand{\bmM}{\ensuremath{\bm M}}
\newcommand{\bmN}{\ensuremath{\bm N}}
\newcommand{\bmO}{\ensuremath{\bm O}}
\newcommand{\bmP}{\ensuremath{\bm P}}
\newcommand{\bmQ}{\ensuremath{\bm Q}}
\newcommand{\bmR}{\ensuremath{\bm R}}
\newcommand{\bmS}{\ensuremath{\bm S}}
\newcommand{\bmT}{\ensuremath{\bm T}}
\newcommand{\bmU}{\ensuremath{\bm U}}
\newcommand{\bmV}{\ensuremath{\bm V}}
\newcommand{\bmW}{\ensuremath{\bm W}}
\newcommand{\bmX}{\ensuremath{\bm X}}
\newcommand{\bmY}{\ensuremath{\bm Y}}
\newcommand{\bmZ}{\ensuremath{\bm Z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                  Probability                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Basic operators and standard notation
\usepackage{amsmath}
\DeclareMathOperator{\pr}{\textsf{P}}
\DeclareMathOperator{\E}{E}
\DeclareMathOperator{\var}{var}
\DeclareMathOperator{\cov}{cov}
\DeclareMathOperator{\sd}{sd}
\DeclareMathOperator{\as}{a.s.}
\DeclareMathOperator{\iid}{\overset{iid}{\sim}}
% Stochastic convergence and stochastic orders
\newcommand{\asto}{\ensuremath{\overset{\mathrm{a.s.}}{\rightarrow}}}
\newcommand{\pto}{\ensuremath{\underset{\mathrm{p}}{\rightarrow}}}
\newcommand{\dto}{\ensuremath{\overset{\mathrm{d}}{\rightarrow}}}
\newcommand{\wto}{\ensuremath{\rightsquigarrow}}
\newcommand{\op}{\ensuremath{o_{\mathrm{p}}(1)}}
\newcommand{\Op}{\ensuremath{O_{\mathrm{p}}(1)}}
% Stochastic processes
\newcommand{\m}{\ensuremath{\overset{\mathrm{m}}{=}}} % equality of marginals
\newcommand{\dd}{\ensuremath{\overset{\mathrm{d}}{=}}} % equality of joints 
\DeclareMathOperator{\GP}{\text{GP}}
\DeclareMathOperator{\DP}{\text{DP}}
\DeclareMathOperator{\PT}{\text{PT}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                  Statistics                                  %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{mathrsfs}
\DeclareMathOperator{\CI}{CI}
\newcommand{\Lik}{\mathscr{L}}
\newcommand{\hatF}{\ensuremath{\widehat{F}}} 
% Distributions
\DeclareMathOperator{\Beta}{Beta}
\DeclareMathOperator{\Bern}{Bern}
\DeclareMathOperator{\Bin}{Bin}
\DeclareMathOperator{\Dir}{Dir}
\DeclareMathOperator{\Exp}{Exp}
\DeclareMathOperator{\Ga}{Gamma}
\DeclareMathOperator{\GEV}{GEV}
\DeclareMathOperator{\GPD}{GPD}
\DeclareMathOperator{\Poi}{Poi}
\DeclareMathOperator{\IG}{IGamma}
\DeclareMathOperator{\U}{Unif}
\DeclareMathOperator{\Weib}{Weibull}
% Probability mass function and densities
\newcommand{\dbeta}[3]{\ensuremath{\frac{1}{B(#2,#3)} #1^{#2 - 1} 
    (1 - #1)^{#3 - 1}}}
\newcommand{\dbern}[2]{\ensuremath{#2^{#1} (1 - #2)^{1 - #1}}}
\newcommand{\dbin}[3]{\ensuremath{\binom{#2}{#1} #3^{#1} (1 - #3)^{#2 - #1}}} 
\newcommand{\ddir}[3]{\ensuremath{\frac{1}{B(\bm{#2})}\prod_{i = 1}^{#3} 
    #1_i^{#2_i - 1}}}
\newcommand{\dexp}[2]{\ensuremath{#2 \exp\lbrace-#2 #1 \rbrace}}
\newcommand{\dexpf}[2]{\ensuremath{\frac{1}{#2} \exp\lbrace -\frac{#1}{#2} 
    \rbrace}}
\newcommand{\dgamma}[3]{\ensuremath{\frac{#3^{#2}}{\Gamma(#2)}{#1}^{#2 - 1}\exp(-#3 #2)}}
\newcommand{\dgammaf}[3]{\ensuremath{\frac{1}{\Gamma{#2}#3^{#2}} #1^{#2 - 1} 
    \exp(-#1/#2)}}
\newcommand{\dnorm}[3]{\ensuremath{\frac{1}{#3\sqrt{2\pi}} 
    \exp\Bigl\lbrace -\frac{1}{2} \Bigl(\frac{#1 - #2}{#3}\Bigr)^2 
    \Bigr\rbrace}}
% Distribution functions
\newcommand{\pexp}[2]{\ensuremath{1 - \exp\lbrace -#2 #1 \rbrace}}
\newcommand{\pgev}[4]{\ensuremath{\exp\bigl[-\Bigl\lbrace 1 + 
    #4 \bigl(\frac{#1 - #2}{#3} \bigr) \Bigr\rbrace^{-1/#4}\bigr]}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                   Computing                                  %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\R}{R}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                               Biostatistics                                  %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DeclareMathOperator{\ROC}{ROC}
\DeclareMathOperator{\AUC}{AUC}
\DeclareMathOperator{\YI}{YI}
\newcommand{\D}{\ensuremath{\bar{D}}}

% % Finance
% \newcommand{\VaR}{\text{VaR}}

% Space
\newcommand{\vs}{\vspace{0.2cm}}
\newcommand{\vS}{\vspace{0.4cm}}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

